The Virtues of Laziness in Model-based RL: A Unified Objective and Algorithms

We propose a novel approach to addressing two fundamental challenges in Model-based Reinforcement Learning (MBRL): the computational expense of repeatedly finding a good policy in the learned model, and the objective mismatch between model fitting and policy computation. Our "lazy" method leverages a novel unified objective, Performance Difference via Advantage in Model, to capture the performance difference between the learned policy and expert policy under the true dynamics. This objective demonstrates that optimizing the expected policy advantage in the learned model under an exploration distribution is sufficient for policy computation, resulting in a significant boost in computational efficiency compared to traditional planning methods. Additionally, the unified objective uses a value moment matching term for model fitting, which is aligned with the model's usage during policy computation. We present two no-regret algorithms to optimize the proposed objective, and demonstrate their statistical and computational gains compared to existing MBRL methods through simulated benchmarks.

==> sections/old.tex <==
\section{Proof for the Realizable Case}

In the model class $\mathcal{M}$, assume there exists a model $\hat{M}$ such that its optimal policy $\hat{\pi}$ achieves both 
zero self-consistency loss, and zero psuedo loss given by:
\begin{align*}
    \mathbb{E}_{(s, a) \sim d_{\omega, \pihat}} \mathbb{E}_{s' \sim M^\star(s, a), s'' \sim \hat{M}(s, a)} |V^{\hat{\pi}}_{\hat{M}}(s') - V^{\hat{\pi}}_{\hat{M}}(s'')| &= 0  && \text{(Self-consistency loss)}\\
    \mathbb{E}_{(s, a) \sim d_{\omega, \pi^\star}} \mathbb{E}_{s' \sim M^\star(s, a), s'' \sim \hat{M}(s, a)} |V^{\hat{\pi}}_{\hat{M}}(s') - V^{\hat{\pi}}_{\hat{M}}(s'')| &= 0 && \text{(Psuedo loss)}
\end{align*}

Given this, we would like to prove that the policy $\hat{\pi}$ achieves the same performance as the optimal policy $\pi^\star$ in the real world $M^\star$.

\begin{theorem}
    Given a model $\hat{M}$ whose optimal policy $\hat{\pi}$ achieves both zero self-consistency loss and zero psuedo loss (as described above), the performance of the policy $\hat{\pi}$ matches that of the expert policy $\pi^\star$ in the real world $M^\star$. In other words,
    \begin{equation}
        \mathbb{E}_{s_0 \sim \omega} V^{\hat{\pi}}_{M^\star}(s_0) = \mathbb{E}_{s_0 \sim \omega} V^{\pi^\star}_{M^\star}(s_0)
    \end{equation}
\end{theorem}
\begin{proof}
    Say, the trajectory $\tau^\star$ taken by $\pi^\star$ in the real world $M^\star$ is given by $s_0, s_1, \cdots, s_{H-1}$. \SAN{Since MDP can be stochastic, there isn't any one trajectory. Instead, the arguments should hold for $s_t$ samples from the state distrib. induced by $\pi^\star$} \ANI{Yes, this theorem assumes deterministic dynamics. The next theorem considers the stochastic setting} We will prove this for the finite horizon case, and the infinite horizon case can be similarly shown. We will ignore the time index on the value functions, and instead use the time index on the states to keep the notation simple.

    We will prove this using the following sequence of arguments:
    \begin{enumerate}
        \item \label{part:1}First, we will show that for all $s_t$ on the optimal trajectory $\tau^\star$, the following holds:
        \begin{equation}
            V^{\hat{\pi}}_{\hat{M}}(s_t) \leq V^{\pi^\star}_{M^\star}(s_t)
        \end{equation}
        \item \label{part:2}Next from self-consistency being zero, we can show that the performance of the policy $\hat{\pi}$ in the model $\hat{M}$ matches its performance in the real world $M^\star$. In other words,
        \begin{equation}
            \mathbb{E}_{s_0 \sim \omega} V^{\hat{\pi}}_{\hat{M}}(s_0) = \mathbb{E}_{s_0 \sim \omega} V^{\hat{\pi}}_{M^\star}(s_0)
        \end{equation}
        \item \label{part:3}Finally, combining the above two results gives us 
        \begin{equation}
        \mathbb{E}_{s_0 \sim \omega} V^{\hat{\pi}}_{M^\star}(s_0) \leq \mathbb{E}_{s_0 \sim \omega} V^{{\pi^\star}}_{M^\star}(s_0)
        \end{equation}
        which can only be true if (since $\pi^\star$ is the optimal policy in $M^\star$)
        \begin{equation}
            \mathbb{E}_{s_0 \sim \omega} V^{\hat{\pi}}_{M^\star}(s_0) = \mathbb{E}_{s_0 \sim \omega} V^{{\pi^\star}}_{M^\star}(s_0)
        \end{equation}
    \end{enumerate}

    Let us start with the first part~\ref{part:1} of the proof. We will prove this through induction from timestep $H-1$ to $0$. To establish the base case, observe that the following is true:
    \begin{equation}
        V_{\hat{M}}^{\hat{\pi}}(s_{H-1}) = V_{M^\star}^{\pi^\star}(s_{H-1})
    \end{equation}
    as $s_{H-1}$ is the terminal state of the horizon. Hence, it satisfies the base case that $V_{\hat{M}}^{\hat{\pi}}(s_{H-1}) \leq V_{M^\star}^{\pi^\star}(s_{H-1})$. 

    Now, let's assume that for some time step $t \in [0, H-1]$, we have 
    \begin{equation}
        V_{\hat{M}}^{\hat{\pi}}(s_{t}) \leq V_{M^\star}^{\pi^\star}(s_{t})
    \end{equation}
    Given this, we would like to prove that $V_{\hat{M}}^{\hat{\pi}}(s_{t-1}) \leq V_{M^\star}^{\pi^\star}(s_{t-1})$. To prove this, observe that we have
    \begin{align*}
        &V_{\hat{M}}^{\hat{\pi}}(s_{t-1}) = \mathbb{E}_{a_{t-1} \sim \hat{\pi}(s_{t-1})}\left[c(s_{t-1}, a_{t-1}) + \mathbb{E}_{\hat{s}_t \sim \hat{M}(s_{t-1}, a_{t-1})}[V_{\hat{M}}^{\hat{\pi}}(\hat{s}_{t})]\right] && \text{(Bellman Eqn)}\\
        &\leq \mathbb{E}_{a_{t-1} \sim \pi^\star(s_{t-1})}\left[c(s_{t-1}, a_{t-1}) + \mathbb{E}_{\hat{s}_t \sim \hat{M}(s_{t-1}, a_{t-1})}[V_{\hat{M}}^{\hat{\pi}}(\hat{s}_{t})]\right] && \text{(Optimality)}\\
        &= \mathbb{E}_{a_{t-1} \sim \pi^\star(s_{t-1})}\left[c(s_{t-1}, a_{t-1}) + \mathbb{E}_{{s}_t \sim {M^\star}(s_{t-1}, a_{t-1})}[V_{\hat{M}}^{\hat{\pi}}({s}_{t})]\right] && \text{(Zero Psuedo loss)} \\
        &\leq \mathbb{E}_{a_{t-1} \sim \pi^\star(s_{t-1})}\left[c(s_{t-1}, a_{t-1}) + \mathbb{E}_{{s}_t \sim {M^\star}(s_{t-1}, a_{t-1})}[V_{{M^\star}}^{{\pi^\star}}({s}_{t})]\right] && \text{(Induction)} \\
        &= V_{M^\star}^{\pi^\star}(s_{t-1})
    \end{align*}
    Note that the second line in the above argument is due to the fact that policy $\hat{\pi}$ is optimal in the model $\hat{M}$. The third line is a direct result of the psuedo loss being zero which implies 
    \begin{equation}
        \mathbb{E}_{(s, a) \sim d_{\omega, \pi^\star}} \mathbb{E}_{s' \sim M^\star(s, a)} V^{\hat{\pi}}_{\hat{M}}(s') = \mathbb{E}_{(s, a) \sim d_{\omega, \pi^\star}} \mathbb{E}_{s'' \sim \hat{M}(s, a)}  V^{\hat{\pi}}_{\hat{M}}(s'')
    \end{equation}
    Finally, the fourth line uses the induction assumption. Note that this is true for any trajectory $\tau^\star$ that the optimal policy $\pi^\star$ can take.
    Thus, we have proved step~\ref{part:1} of the proof.

    On to proving step~\ref{part:2} of the proof. From simulation lemma we have,
    \begin{align*}
        \mathbb{E}_{s_0 \sim \omega}[V_{M^\star}^{\hat{\pi}}(s_0) - V_{\hat{M}}^{\hat{\pi}}(s_0)] &= \mathbb{E}_{(s, a) \sim d_{\omega, \pihat}} \mathbb{E}_{s' \sim M^\star(s, a), s'' \sim \hat{M}(s, a)} [V^{\hat{\pi}}_{\hat{M}}(s') - V^{\hat{\pi}}_{\hat{M}}(s'')] \\
        &\leq \mathbb{E}_{(s, a) \sim d_{\omega, \pihat}} \mathbb{E}_{s' \sim M^\star(s, a), s'' \sim \hat{M}(s, a)} |V^{\hat{\pi}}_{\hat{M}}(s') - V^{\hat{\pi}}_{\hat{M}}(s'')| && \\
        &= 0
    \end{align*}
    the last line follows from the fact that self-consistency loss is zero. Hence, we have that
    \begin{equation}
        \mathbb{E}_{s_0 \sim \omega} V^{\hat{\pi}}_{\hat{M}}(s_0) = \mathbb{E}_{s_0 \sim \omega} V^{\hat{\pi}}_{M^\star}(s_0)
    \end{equation}
    and step~\ref{part:2} is proved.

    Step~\ref{part:3} requires combining step~\ref{part:1} and step~\ref{part:2}. By combining the previous results, we have 
    \begin{equation}
        \mathbb{E}_{s_0 \sim \omega} V^{\hat{\pi}}_{M^\star}(s_0) = \mathbb{E}_{s_0 \sim \omega} V^{\hat{\pi}}_{\hat{M}}(s_0) \leq \mathbb{E}_{s_0 \sim \omega} V^{\pi^\star}_{M^\star}(s_0)
    \end{equation}

    But policy $\pi^\star$ is optimal in the real world $M^\star$, so the inequality must be tight resulting in
    \begin{equation}
        \mathbb{E}_{s_0 \sim \omega} V^{\hat{\pi}}_{M^\star}(s_0) = \mathbb{E}_{s_0 \sim \omega} V^{\pi^\star}_{M^\star}(s_0)
    \end{equation}
    Hence, the performance of the policy $\hat{\pi}$ in the real world $M^\star$ matches that of the optimal policy $\pi^\star$.
\end{proof}

\section{Proof for the Agnostic Case}

In the model class $\mathcal{M}$, assume there exists a model $\Mhat$ such that its optimal policy $\pihat$ achieves the following:
\begin{align*}
    &\mathbb{E}_{(s, a) \sim d_{\omega, \pihat}}\mathbb{E}_{s' \sim \Mstar(s, a), s'' \sim \Mhat(s, a)}|V_{\Mhat}^{\pihat}(s') - V_{\Mhat}^{\pihat}(s'')| \leq \epsilon && \text{(Self-consistency loss)} \\
    &\mathbb{E}_{(s, a) \sim d_{\omega, \pistar}}\mathbb{E}_{s' \sim \Mstar(s, a), s'' \sim \Mhat(s, a)}|V_{\Mhat}^{\pihat}(s') - V_{\Mhat}^{\pihat}(s'')| \leq \epsilon && \text{(Psuedo loss)}
\end{align*}
Given this, we would like to prove that the policy $\pihat$ achieves a bounded suboptimal performance when compared to the optimal policy $\pistar$ in the real world $\Mstar$.

\begin{theorem}
    Given a model $\Mhat$ whose optimal policy $\pihat$ achieves self-consistency loss and psuedo loss (both) bounded by $\epsilon \in \mathbb{R}^+$, then the performance of the policy $\pihat$ in real world $\Mstar$ is bounded above as follows:
    \begin{equation}
        \mathbb{E}_{s_0 \sim \omega} V^{\pihat}_{\Mstar}(s_0) \leq \mathbb{E}_{s_0 \sim \omega} V^{\pistar}_{\Mstar}(s_0) + H\epsilon
    \end{equation}
    where $H$ is the horizon.
\end{theorem}
\begin{proof}
    For ease of notation, we will ignore the time index on the value functions, and instead use the time index on the states to keep the notation simple.
    
    We will prove this using the following sequence of arguments:
    \begin{enumerate}
        \item\label{ref:agnostic-part-1} First, we will show that the following holds:
        \begin{equation}
            \mathbb{E}_{s_t \sim d_{\omega, \pistar}^t} V_{\Mhat}^{\pihat}(s_t) \leq \mathbb{E}_{s_t \sim d_{\omega, \pistar}^t} V_{\Mstar}^{\pistar}(s_t) + (H-t-1)\epsilon
        \end{equation}
        where $d_{\omega, \pistar}^t$ is the distribution of states at time $t$ if we execute policy $\pistar$ until time $t-1$ starting from a state sampled from distribution $\omega$.
        \item\label{ref:agnostic-part-2} Next, using the fact that self-consistency loss is bounded, we will show that the performance of the policy $\pihat$ in the model $\Mstar$ is bounded above as follows:
        \begin{equation}
            \mathbb{E}_{s_0 \sim \omega} V_{\Mstar}^{\pihat}(s_0) \leq \mathbb{E}_{s_0 \sim \omega} V_{\Mhat}^{\pihat}(s_0) + \epsilon
        \end{equation}
        \item\label{ref:agnostic-part-3} Finally, combining the above two results gives us
        \begin{equation}
            \mathbb{E}_{s_0 \sim \omega} V_{\Mstar}^{\pihat}(s_0) \leq \mathbb{E}_{s_0 \sim \omega} V_{\Mstar}^{\pistar}(s_0) + H\epsilon
        \end{equation}
    \end{enumerate}
    
    Let us start with the first part~\ref{ref:agnostic-part-1} of the proof. We will prove this through induction from timestep $H-1$ to $0$. To establish the base case, observe that the following is true:
    \begin{equation}
        \mathbb{E}_{s_{H-1} \sim d_{\omega, \pistar}^{H-1}} V_{\Mhat}^{\pihat}(s_{H-1}) = \mathbb{E}_{s_{H-1} \sim d_{\omega, \pistar}^{H-1}} V_{\Mstar}^{\pistar}(s_{H-1})
    \end{equation}
    as $s_{H-1}$ is the terminal state of the horizon. Hence, it satisfies the base case that $\mathbb{E}_{s_{H-1} \sim d_{\omega, \pistar}^{H-1}} V_{\Mhat}^{\pihat}(s_{H-1}) \leq \mathbb{E}_{s_{H-1} \sim d_{\omega, \pistar}^{H-1}} V_{\Mstar}^{\pistar}(s_{H-1})$.
    
    Now, let's assume that for some time step $t \in [0, H-1]$, we have
    \begin{equation}
        \mathbb{E}_{s_t \sim d_{\omega, \pistar}^t} V_{\Mhat}^{\pihat}(s_t) \leq \mathbb{E}_{s_t \sim d_{\omega, \pistar}^t} V_{\Mstar}^{\pistar}(s_t) + (H-t-1)\epsilon
    \end{equation}
    Given this, we would like to prove that 
    \begin{equation}
    \mathbb{E}_{s_{t-1} \sim d_{\omega, \pistar}^{t-1}} V_{\Mhat}^{\pihat}(s_{t-1}) \leq \mathbb{E}_{s_{t-1} \sim d_{\omega, \pistar}^{t-1}} V_{\Mstar}^{\pistar}(s_{t-1}) + (H-t)\epsilon
    \end{equation}
    To prove this, observe that we have
    \begin{align*}
        &\mathbb{E}_{s_{t-1} \sim d_{\omega, \pistar}^{t-1}} V_{\Mhat}^{\pihat}(s_{t-1}) = \mathbb{E}_{s_{t-1} \sim d_{\omega, \pistar}^{t-1}, a_{t-1} \sim \pihat(s_{t-1})}\left[ c(s_{t-1}, a_{t-1}) + \mathbb{E}_{\hat{s}_t \sim \Mhat(s_{t-1}, a_{t-1})} V^{\pihat}_{\Mhat}(\hat{s}_t)\right] && \text{(Bellman eqn)}\\
        &\leq \mathbb{E}_{s_{t-1} \sim d_{\omega, \pistar}^{t-1}, a_{t-1} \sim \pistar(s_{t-1})}\left[ c(s_{t-1}, a_{t-1}) + \mathbb{E}_{\hat{s}_t \sim \Mhat(s_{t-1}, a_{t-1})} V^{\pihat}_{\Mhat}(\hat{s}_t)\right] && \text{(Opt of $\pihat$ in $\Mhat$)} \\
        &= \mathbb{E}_{(s_{t-1}, a_{t-1}) \sim d_{\omega, \pistar}}[c(s_{t-1}, a_{t-1})] + \mathbb{E}_{(s_{t-1}, a_{t-1}) \sim d_{\omega, \pistar}} \mathbb{E}_{\hat{s}_t \sim \Mhat(s_{t-1}, a_{t-1})} V^{\pihat}_{\Mhat}(\hat{s}_t) && \\
        &\leq \mathbb{E}_{(s_{t-1}, a_{t-1}) \sim d_{\omega, \pistar}}[c(s_{t-1}, a_{t-1})] + \mathbb{E}_{(s_{t-1}, a_{t-1}) \sim d_{\omega, \pistar}} \mathbb{E}_{s_t \sim \Mstar(s_{t-1}, a_{t-1})} V^{\pihat}_{\Mhat}(s_t) + \epsilon && \text{(Psuedo loss)} \\
        &=  \mathbb{E}_{(s_{t-1}, a_{t-1}) \sim d_{\omega, \pistar}}[c(s_{t-1}, a_{t-1})] + \mathbb{E}_{s_t \sim d_{\omega, \pistar}^t} V^{\pihat}_{\Mhat}(s_t) + \epsilon && \\
        &\leq \mathbb{E}_{(s_{t-1}, a_{t-1}) \sim d_{\omega, \pistar}}[c(s_{t-1}, a_{t-1})] + \mathbb{E}_{s_t \sim d_{\omega, \pistar}^t} V^{\pistar}_{\Mstar}(s_t) + (H-t-1)\epsilon + \epsilon && \text{(Induction)} \\
        &= \mathbb{E}_{(s_{t-1}, a_{t-1}) \sim d_{\omega, \pistar}}[c(s_{t-1}, a_{t-1})] + \mathbb{E}_{(s_{t-1}, a_{t-1}) \sim d_{\omega, \pistar}} \mathbb{E}_{s_t \sim \Mstar(s_{t-1}, a_{t-1})} V^{\pistar}_{\Mstar}(s_t) + (H-t)\epsilon && \\
        &= \mathbb{E}_{(s_{t-1}, a_{t-1}) \sim d_{\omega, \pistar}} \left[ c(s_{t-1}, a_{t-1}) + \mathbb{E}_{s_t \sim \Mstar(s_{t-1}, a_{t-1})} V^{\pistar}_{\Mstar}(s_t) \right] + (H-t)\epsilon && \\
        &= \mathbb{E}_{s_{t-1} \sim d_{\omega, \pistar}^{t-1}, a_{t-1} \sim \pistar(s_{t-1})}\left[ c(s_{t-1}, a_{t-1}) + \mathbb{E}_{s_t \sim \Mstar(s_{t-1}, a_{t-1})} V^{\pistar}_{\Mstar}(s_t) \right] + (H-t)\epsilon && \\
        &= \mathbb{E}_{s_{t-1} \sim d_{\omega, \pistar}^{t-1}} V^{\pistar}_{\Mstar}(s_{t-1}) + (H-t)\epsilon && \text{(Bellman eqn)}
    \end{align*}
    Thus, we have proved step~\ref{ref:agnostic-part-1} of the proof.
    
    On to proving step~\ref{ref:agnostic-part-2} of the proof. From simulation lemma we have,
    \begin{align*}
        \mathbb{E}_{s_0 \sim \omega}[V_{M^\star}^{\hat{\pi}}(s_0) - V_{\hat{M}}^{\hat{\pi}}(s_0)] &= \mathbb{E}_{(s, a) \sim d_{\omega, \pihat}} \mathbb{E}_{s' \sim M^\star(s, a), s'' \sim \hat{M}(s, a)} [V^{\hat{\pi}}_{\hat{M}}(s') - V^{\hat{\pi}}_{\hat{M}}(s'')] \\
        &\leq \mathbb{E}_{(s, a) \sim d_{\omega, \pihat}} \mathbb{E}_{s' \sim M^\star(s, a), s'' \sim \hat{M}(s, a)} |V^{\hat{\pi}}_{\hat{M}}(s') - V^{\hat{\pi}}_{\hat{M}}(s'')| && \\
        &\leq \epsilon
    \end{align*}
    the last line follows from the fact that self-consistency loss is bounded above by $\epsilon$. Hence, we have that
    \begin{equation}
        \mathbb{E}_{s_0 \sim \omega} V_{\Mstar}^{\pihat}(s_0) \leq \mathbb{E}_{s_0 \sim \omega} V_{\Mhat}^{\pihat}(s_0) + \epsilon
    \end{equation}
    and step~\ref{ref:agnostic-part-2} is proved.
    
    Step~\ref{ref:agnostic-part-3} requires combining step~\ref{ref:agnostic-part-1} and step~\ref{ref:agnostic-part-2}. From step~\ref{ref:agnostic-part-1}, we have at time step $0$:
    \begin{align}
        \mathbb{E}_{s_0 \sim d_{\omega, \pistar}^0} V_{\Mhat}^{\pihat}(s_0) &\leq \mathbb{E}_{s_0 \sim d_{\omega, \pistar}^0} V_{\Mstar}^{\pistar}(s_0) + (H-1)\epsilon \\
        \mathbb{E}_{s_0 \sim \omega} V_{\Mhat}^{\pihat}(s_0) &\leq \mathbb{E}_{s_0 \sim \omega} V_{\Mstar}^{\pistar}(s_0) + (H-1)\epsilon
    \end{align}
    since $d_{\omega, \pistar}^0 = \omega$. Combining this with result of step~\ref{ref:agnostic-part-2} we get:
    \begin{equation}
            \mathbb{E}_{s_0 \sim \omega} V_{\Mstar}^{\pihat}(s_0) \leq \mathbb{E}_{s_0 \sim \omega} V_{\Mstar}^{\pistar}(s_0) + H\epsilon
        \end{equation}
        
\end{proof}


\iffalse

\section{Latent Simulation Lemma}
Let's first introduce notation: denote $V: \Scal \to \RR$ as the normal value function such that $V^{\pi}_{M^{\ast}}(s) = \EE \left[ \sum_{h=0}^{\infty} \gamma^h R(s_h,a_h) \mid s_0 = s, a_h \sim \pi(s_h), s_{h+1} \sim M^{\ast}(s_h,a_h) \right]$. To avoid conflicted notation, let's use $z$ instead of $h$ for the latent/hidden state, and $\Zcal$ as the latent state space. Let $\phi: \Scal \to \Zcal$ denotes the encoder that maps from observation/state space $\Scal$ to the latent/hidden space $\Zcal$. We use $\tilde{}$ to denote everything that learned in the latent: for example, let $\tilde R: \Zcal \times \Acal \to \RR$ be the learned latent reward function, and $\tilde M: \Zcal \times \Acal \to \Delta(\Zcal)$ be the learned latent dynamics. Let $\tilde M^\phi: \Scal \times \Acal \to \Delta(\Zcal)$ be the latent model equipped with encoder $\phi$ such that $\tilde M^\phi(s,a) = \tilde M (\phi(s),a)$. Denote the latent value function as $\tilde V: \Zcal \to \RR$, and $\tilde V^{\pi}_{\tilde M}(z) = \EE \left[ \sum_{h=0}^{\infty} \gamma^h R(z_h,a_h) \mid z_0 = z, a_h \sim \pi(z), z_{h+1} \sim M^{\ast}(z_h,a_h) \right]$.

Now let's introduce some weird notation: Let $\tilde V^{\pi}_{\tilde M, \phi}: \Scal \times \Acal \to \RR$ be the value of the latent policy in the latent model but evaluated on the real state, i.e., $\tilde V^{\pi}_{\tilde M, \phi}(s) = \EE_{a \sim \pi(\phi(s))}\left[\tilde R(\phi(s),a) + \gamma \EE_{h' \sim \tilde M(\phi(s),a)} \tilde V^{\pi}_{\tilde M}(h')\right]$. With this we can proceed.

So let's try to bound (with slight abuse of notation that $\pi$ operates both on $\Scal$ (with $\phi$) and $\Zcal$):
\begin{align*}
    \EE_{s \sim d_0}\left[ V^{\pi}_{M^{\ast}}(s) - \tilde V^{\pi}_{\tilde M, \phi}(s) \right] &= \EE_{s \sim d_0} \EE_{a \sim \pi(s)} \left[R(s,a) + \gamma \EE_{s' \sim M^{\ast}(s,a)}[V^{\pi}_{M^{\ast}}(s')] - \tilde R(\phi(s),a) - \gamma\EE_{z' \sim \tilde M(\phi(s),a)}[\tilde V^{\pi}_{\tilde M, \phi}(z')] \right] \\
    &= \EE_{s,a \sim d_0^{\pi}} \Bigl[R(s,a) - \tilde R(\phi(s),a) + \underbrace{\gamma \EE_{s' \sim M^{\ast}(s,a)}[V^{\pi}_{M^{\ast}}(s')] - \gamma \EE_{s' \sim M^{\ast}(s,a)}[\tilde V^{\pi}_{\tilde M, \phi}(s')]}_{Re} \\ & \quad + \gamma \EE_{s' \sim M^{\ast}(s,a)}[\tilde V^{\pi}_{\tilde M, \phi}(s')]   -\EE_{z' \sim \tilde M(\phi(s),a)}[\tilde V^{\pi}_{\tilde M}(z')] \Bigr]
\end{align*}
Then recursively expanding on $Re$ gives
\begin{align*}
    \EE_{s \sim d_0}\left[ V^{\pi}_{M^{\ast}}(s) - \tilde V^{\pi}_{\tilde M, \phi}(s) \right] &= \frac{\gamma}{1-\gamma}\EE_{s,a \sim d^{\pi}}  \left[ R(s,a) - \tilde R(\phi(s),a) + \EE_{s' \sim M^{\ast}(s,a)}[\tilde V^{\pi}_{\tilde M, \phi}(s')]   -\EE_{z' \sim \tilde M(\phi(s),a)}[\tilde V^{\pi}_{\tilde M}(z')] \right]
\end{align*}
Now let's consider some strange construction $M^{\ast}_{\phi}: \Scal \times \Acal \to \Delta(\Zcal)$ with that construction $M^{\ast}_{\phi}(s,a) = (\phi \circ M^{\ast})(s,a)$. This is valid if $\phi$ is $\Scal/\Zcal$-measurable (sorry Drew...), for example, continuous? And then we can do something like:
\begin{align*}
    \EE_{s \sim d_0}\left[ V^{\pi}_{M^{\ast}}(s) - \tilde V^{\pi}_{\tilde M, \phi}(s) \right] &= \frac{\gamma}{1-\gamma}\EE_{s,a \sim d^{\pi}}  \left[ R(s,a) - \tilde R(\phi(s),a) + \EE_{z' \sim M^{\ast}_{\phi}(s,a)}[\tilde V^{\pi}_{\tilde M}(z')]   -\EE_{z' \sim \tilde M(\phi(s),a)}[\tilde V^{\pi}_{\tilde M}(z')] \right]
\end{align*}
and then we can do holder? 

Another way is to think of there exists some decoder function $\psi$ such that $(\psi \circ \tilde M_{\phi})(s,a)$ is always a probability measure on $\Scal$ for all $s,a$?

Extending the result to the double simulation lemma is straight forward:n we have 
\begin{align*}
        \mathbb{E}_{s \sim d_0} [V_{M^\star}^{\hat{\pi}}(s) - V_{M^\star}^{\pi^\star}(s)] =&  \mathbb{E}_{s \sim d_0}\left[ (V^{\pihat}_{\Mhat}(s) - V_{\Mhat}^{\pistar}(s)) + (V^{\pihat}_{\Mstar}(s) - V^{\pihat}_{\Mhat}(s)) + (V^{\pistar}_{\Mhat}(s) - V^{\pistar}_{\Mstar}(s))\right] \\
        \leq& \underbrace{\mathbb{E}_{s \sim d_0}\left[ V^{\pihat}_{\Mhat}(s) - V_{\Mhat}^{\pistar}(s)\right]}_{\leq 0}  \\
        & + \frac{\gamma}{1-\gamma}\EE_{s,a \sim d^{\hat \pi}}  \left[ R(s,a) - \tilde R(\phi(s),a) + \EE_{z' \sim M^{\ast}_{\phi}(s,a)}[\tilde V^{\hat \pi}_{\tilde M, \phi}(z')]   -\EE_{z' \sim \tilde M(\phi(s),a)}[\tilde V^{\hat \pi}_{\tilde M}(z')] \right] \\
        & + \frac{\gamma}{1-\gamma}\EE_{s,a \sim d^{ \pi^{\ast}}}   \left[ \tilde R(\phi(s),a) - R(s,a)  +   \EE_{s' \sim \tilde M_{\psi}(\phi(s),a)}[V^{\pi^{\ast}}_{M^{\ast}}(s')] - \EE_{s' \sim M^{\ast}(s,a)}[ V^{\pi^{\ast}}_{M^{\ast}}(s')]\right].
\end{align*}
This double simulation lemma may justify the need for learning a decoder...\\
But let's next see what happens when we use performance PDL: we use
\begin{align*}
    \mathbb{E}_{s \sim d_0} [V_{M^\star}^{\hat{\pi}}(s) - V_{M^\star}^{\pi^\star}(s)] =& \EE_{s \sim d_0}\left[V^{\hat \pi}_{M^{\ast}}(s) - V^{\hat \pi}_{\tilde M}(s)\right] + \EE_{s \sim d_0}\left[V^{\hat \pi}_{\tilde M}(s) - V_{M^\star}^{\pi^\star}(s)\right].
\end{align*}
First term is latent simulation lemma, let's bound the second term.
We have:
\begin{align*}
     \EE_{s \sim d_0}\left[V^{\hat \pi}_{\tilde M}(s) - V_{M^\star}^{\pi^\star}(s)\right] &= \EE_{s \sim d_0}\left[V^{\hat \pi}_{\tilde M}(s) -\EE_{a\sim \pi^{\ast}} Q^{\hat \pi}_{\tilde M}(s,a) + \EE_{a\sim \pi^{\ast}} Q^{\hat \pi}_{\tilde M}(s,a) - V_{M^\star}^{\pi^\star}(s)\right] \\
     &= \EE_{s \sim d_0}\left[V^{\hat \pi}_{\tilde M}(s) -\EE_{a\sim \pi^{\ast}} Q^{\hat \pi}_{\tilde M}(s,a)\right] \\&\quad+ \EE_{s,a \sim d^{\pi^{\ast}}} \left[  \tilde R(\phi(s),a) + \gamma \EE_{z' \sim \tilde M(s,a)} V^{\hat \pi}_{\tilde M}(z') - R(s,a) + \gamma \EE_{s' \sim M^{\ast}}  V_{M^\star}^{\pi^\star}(s')\right] \\
     &= \EE_{s \sim d_0}\left[V^{\hat \pi}_{\tilde M}(s) -\EE_{a\sim \pi^{\ast}} Q^{\hat \pi}_{\tilde M}(s,a)\right] \\&\quad+ \EE_{s,a \sim d^{\pi^{\ast}}_0} \left[  \tilde R(\phi(s),a) - R(s,a)\right] \\&\quad+ \gamma \EE_{s,a \sim d^{\pi^{\ast}}_0}\left[\EE_{z' \sim \tilde M(s,a)} V^{\hat \pi}_{\tilde M}(z') -  \EE_{s' \sim M^{\ast}(s,a)} V^{\hat \pi}_{\tilde M}(s') + \EE_{s' \sim M^{\ast}(s,a)} V^{\hat \pi}_{\tilde M}(s') -  \EE_{s' \sim M^{\ast}}  V_{M^\star}^{\pi^\star}(s')\right]
     &= \EE_{s \sim d_0}\left[V^{\hat \pi}_{\tilde M}(s) -\EE_{a\sim \pi^{\ast}} Q^{\hat \pi}_{\tilde M}(s,a)\right] \\&\quad+ \EE_{s,a \sim d^{\pi^{\ast}}_0} \left[  \tilde R(\phi(s),a) - R(s,a)\right] \\&\quad+ \gamma \EE_{s,a \sim d^{\pi^{\ast}}_0}\left[\EE_{z' \sim \tilde M(s,a)} V^{\hat \pi}_{\tilde M}(z') -  \EE_{z' \sim M^{\ast}_{\phi}(s,a)} V^{\hat \pi}_{\tilde M}(z') + \underbrace{\EE_{s' \sim M^{\ast}(s,a)} V^{\hat \pi}_{\tilde M}(s') -  \EE_{s' \sim M^{\ast}}  V_{M^\star}^{\pi^\star}(s')}_{Re}\right],
\end{align*}
and now recursively expanding on $Re$ gives us
\begin{align*}
    \EE_{s \sim d_0}\left[V^{\hat \pi}_{\tilde M}(s) - V_{M^\star}^{\pi^\star}(s)\right] =& \frac{1}{1-\gamma}\EE_{s,a \sim d^{\pi^{\ast}}} \left[V^{\hat \pi}_{\tilde M}(s) - Q^{\hat \pi}_{\tilde M}(s,a)\right]\\ &+ \frac{\gamma}{1-\gamma}\EE_{s,a \sim d^{\pi^{\ast}}}\left[ R(\phi(s),a) - R(s,a) + \EE_{z' \sim \tilde M(s,a)} V^{\hat \pi}_{\tilde M}(z') -  \EE_{z' \sim M^{\ast}_{\phi}(s,a)} V^{\hat \pi}_{\tilde M}(z')\right].
\end{align*}
We can see that in this decomposition we don't need the decoder $\psi$!
\fi

